See through Gradients: Image Batch Recovery via GradInversion

Training deep neural networks requires gradient estimation from data batches to update parameters. Gradients per parameter are averaged over a set of data and this has been presumed to be safe for privacy-preserving training in joint, collaborative, and federated learning applications. Prior work only showed the possibility of recovering input data given gradients under very restrictive conditions - a single input point, or a network with no non-linearities, or a small 32x32 px input batch. Therefore, averaging gradients over larger batches was thought to be safe. In this work, we introduce GradInversion, using which input images from a larger batch (8 - 48 images) can also be recovered for large networks such as ResNets (50 layers), on complex datasets such as ImageNet (1000 classes, 224x224 px). We formulate an optimization task that converts random noise into natural images, matching gradients while regularizing image fidelity. We also propose an algorithm for target class label recovery given gradients. We further propose a group consistency regularization framework, where multiple agents starting from different random seeds work together to find an enhanced reconstruction of original data batch. We show that gradients encode a surprisingly large amount of information, such that all the individual images can be recovered with high fidelity via GradInversion, even for complex datasets, deep networks, and large batch sizes.

==> acknowledgement.tex <==
\section*{Acknowledgments}
Anonymous CVPR submission.

==> application_knowledge_transfer.tex <==



%% Arun edited.
In this section, we show that we can distill information from a teacher network to a student network without using any real images at all. We apply DeepInversion to a ResNet50v1.5~\cite{resnet50v15url} trained on ImageNet to synthesize images. Using these images, we then train another randomly initialized ResNet50v1.5 from scratch. Below, we describe two practical considerations: a) image clipping, and b) multi-resolution synthesis, which we find can greatly help boost accuracy while reducing run-time. A set of images generated by DeepInversion on the pretrained ResNet50v1.5 is shown in Fig.~\ref{fig:resnetv1.5}. The images demonstrate high fidelity and diversity. %Clipping helps improve the contrast, while multi-resolution synthesis helps speed up the process.

\noindent\textbf{a) Image clipping.} 
%\Danny{@Pavlo - shall we shorten here?}\ZL{This can be shortened to: We find that clipping the images to realistic values (0-1 prior to the input normalization used by all networks) helps improve accuracy. Note that the mean and variance here comes from the pre-processing step, which all released models must provide. Since we generate post-normalization images, we clip the  synthesized image $\hat{x}$ using}
We find that enforcing the synthesized images to conform to the mean and variance of the data preprocessing step helps improve accuracy. Note that commonly released networks use means and variances computed on ImageNet. 
%We would like to emphasize that our method does not require statistics of prior datasets, but merely uses those provided with the model, such as the preprocessing statistics. 
We clip synthesized images to be in the $[-m / s, m / s ]$ range, with $m$ representing the per channel mean, and $s$ per channel standard deviation. 
% We clip the synthesized image $\hat{x}$ using
% \vspace{-2mm}
% \begin{eqnarray}
%     \hat{x} & = & \min\big(\max(\hat{x}, -m / s ), (1 - m) / s\big),
% \end{eqnarray}
% where $m=\{0.485, 0.456, 0.406\}$ and $s=$ $\{0.229,$ $ 0.224, $ $0.225\}$. 
% Clipping helps limit the value ranges of pixels and improve contrast, while the color channel means and variances are typically easy to be acquired without breaching the security concern.

\begin{comment}
\begin{figure}
\centering
\includegraphics[width=0.48\textwidth]{figures/imagenet_rn50v15/294.png}
\includegraphics[width=0.48\textwidth]{figures/imagenet_rn50v15/749.png}
\includegraphics[width=0.48\textwidth]{figures/imagenet_rn50v15/874.png}
% \includegraphics[width=\textwidth]{figures/imagenet_rn50v15/890.png}
% \includegraphics[width=\textwidth]{figures/imagenet_rn50v15/907.png}
%\includegraphics[width=0.48\textwidth]{figures/imagenet_rn50v15/915.png}
\includegraphics[width=0.48\textwidth]{figures/imagenet_rn50v15/933.png}
\includegraphics[width=0.48\textwidth]{figures/imagenet_rn50v15/968.png}
\includegraphics[width=0.48\textwidth]{figures/imagenet_rn50v15/980.png}
\includegraphics[width=0.48\textwidth]{figures/imagenet_rn50v15/985.png}
\includegraphics[width=0.48\textwidth]{figures/imagenet_rn50v15/946.png}
%\caption{Example of inverted images from ResNet50v1.5 by our method. Classes top to bottom: brown bear, quill, trolleybus, yurt, cheeseburger, cup, volcano, daisy, cardoon.}
\caption{Class-conditional $224\times224$ images by DeepInversion given a ResNet50v1.5 classifier pretrained on ImageNet. Classes top to bottom: brown bear, quill, trolleybus, cheeseburger, cup, volcano, daisy, cardoon. %\Danny{@Pavlo: Shall we show fewer but larger images per row to fit in one column? Open to jointly arrange this with Fig. 5.}
}
\vspace{-1mm}
\label{fig:resnetv1.5}
\end{figure}
%\vspace{-3mm}
\end{comment}


\begin{figure}
\centering
\includegraphics[width=0.48\textwidth]{figures/imagenet_rn50v15/fig6_3.pdf}
% \includegraphics[width=0.48\textwidth]{figures/imagenet_rn50v15/294_red.jpg}
% \includegraphics[width=0.48\textwidth]{figures/imagenet_rn50v15/749_red.jpg}
% \includegraphics[width=0.48\textwidth]{figures/imagenet_rn50v15/874_red.jpg}
% \includegraphics[width=0.48\textwidth]{figures/imagenet_rn50v15/933_red.jpg}
% \includegraphics[width=0.48\textwidth]{figures/imagenet_rn50v15/968_red.jpg}
% \includegraphics[width=0.48\textwidth]{figures/imagenet_rn50v15/980_red.jpg}
% \includegraphics[width=0.48\textwidth]{figures/imagenet_rn50v15/985_red.jpg}
% \includegraphics[width=0.48\textwidth]{figures/imagenet_rn50v15/946_red.jpg}
%\caption{Example of inverted images from ResNet50v1.5 by our method. Classes top to bottom: brown bear, quill, trolleybus, yurt, cheeseburger, cup, volcano, daisy, cardoon.}
\caption{Class-conditional $224\times224$ images obtained by DeepInversion given a ResNet50v1.5 classifier pretrained on ImageNet. Classes top to bottom: (left) daisy, volcano, quill, (right) cheeseburger, brown bear, trolleybus. 
}
\vspace{-1mm}
\label{fig:resnetv1.5}
\end{figure}
%\vspace{-3mm}

\noindent\textbf{b) Multi-resolution synthesis.} We find that we can speed up DeepInversion by employing a multi-resolution optimization scheme. We first optimize the input of resolution $112\times112$ for $2$k iterations. Then, we up-sample the image via nearest neighbor interpolation to $224\times224$, and then optimize for an additional $1$k iterations. This speeds up DeepInversion to $84$ images per $6$ minutes on an NVIDIA V100 GPU. Hyperparameters %for this experiment 
are given in the Appendix. %\Danny{from here on-wards, cut and moved to suppl.} We use the following parameters for this experiment: $\alpha_{\text{tv}}=1\cdot 10^{-4}$, $\alpha_{f}=0.01$, and a learning rate of $0.2$ for Adam. As a final setup, we generate images with an equal probability between this (i) multi-resolution scheme and (ii) the scheme described in Section~\ref{sec:imagenet_deepinversion} with $2$k iterations only to further improve image diversity.

% \noindent\textbf{Sample images.} 


\noindent\textbf{Knowledge transfer.} We synthesize 140k images via DeepInversion on ResNet50v1.5~\cite{resnet50v15url} to train a student network with the same architecture from scratch. Our teacher is a %PyTorch 
pretrained ResNet50v1.5 that achieves $77.26\%$ top-1 accuracy. We apply knowledge distillation for 90/250 epochs, with temperature $\tau=3$, initial learning rate of $1.024$, batch size of $1024$ split across eight V100 GPUs, and other settings the same as in the original setup~\cite{resnet50v15url}. Results are summarized in Table~\ref{tab:resnet50v15_scratch}. The proposed method, given only the trained ResNet50v1.5 model, can teach a new model from scratch to achieve a $73.8\%$ accuracy, which is only $3.46\%$ below the accuracy of the teacher.  

%Performing knowledge distillation with only inverted images results in $64.9\%$ accuracy (top-1). We compare this result to 215k images generated with BigGAN - $64.0\%$, and to 215k randomly selected images from ImageNet - $76.1\%$. Results indicate that our synthesized images are well suited for knowledge distillation to a new student, where we even observe improvements over BigGAN images. Despite a high final accuracy, there still remains room for improvement.
% between distilling with synthesized images and original ones. 
%\pmnote{to update numbers and give conclusion, probably table.}
%\Danny{shall we explain ADI too here? Later pruning can just refer here as 'we use the previously generated images?' But might hard to justify students as ResNet but not v1.5.}
%\Danny{to move later}
% ImageNet & 76.1\\
% BigGan & 64.0\\
% Adaptive & \multirow{2}{*}{64.9}\\
\input{tables/resnet50v15_scratch.tex}

==> discussions.tex <==
%\section*{Discussions}

%One major observation lies in that a trained CNN classifier can already support generating natural images. With a widespread usage of CNNs in addition to the classification application, this observation hints on the potential to inverse pretrained CNNs for more types of inputs: videos, point clouds, segmentation masks, etc. The method may even scale to other network architectures, \textit{e.g.} LSTMs: potential sequential inputs may be reversed given gradients from a pretrained model governed by domain-specific priors, \textit{e.g.} frequency regularization for speech.


==> figures/ablation_col.tex <==
\begin{figure}[t]
\centering

\resizebox{\linewidth}{!}{
\begingroup
% \renewcommand*{\arraystretch}{0.3}
% \setlength\extrarowheight{-30pt}
\begin{tabular}{cc}
% grad only
A & \includegraphics[width=\linewidth]{figures/ablation_images/grad_only.jpg} \\

\tiny{B} & \includegraphics[width=\linewidth]{figures/ablation_images/1gpu.jpg} \\

\tiny{C} & \includegraphics[width=\linewidth]{figures/ablation_images/4gpu_mean.jpg} \\

\tiny{D} & \includegraphics[width=\linewidth]{figures/ablation_images/4gpu_reg2.jpg} \\

\tiny{$\mathbf{x^*}$} & \includegraphics[width=\linewidth]{figures/ablation_images/original.jpg} \\
 \vspace{1mm} \\
\end{tabular}
\endgroup
}
\caption{ImageNet batch gradient inversion for ResNet-50 visual comparison for ablation study.}
\label{fig:against_sota}
\end{figure}


==> figures/main_results_image.tex <==
% \begin{figure*}
% \begin{multicols}{5}
%     \includegraphics[width=\linewidth]{figures/ablation_images/original.jpg}\par 
%     \includegraphics[width=\linewidth]{figures/ablation_images/grad_only.jpg}\par 
%     \includegraphics[width=\linewidth]{figures/ablation_images/1gpu.jpg}\par 
%     \includegraphics[width=\linewidth]{figures/ablation_images/4gpu_mean.jpg}\par 
%     \includegraphics[width=\linewidth]{figures/ablation_images/4gpu_reg.jpg}\par 
%     \end{multicols}
% \caption{Towards the inversion of original batch of resolution $224\times224$ on ImageNet. (preliminary: will format into single rows.)}
% \label{fig:main_results_image}
% \end{figure*}

% \begin{figure*}
% \centering
%  \begin{subfigure}[width=.95\linewidth]
%     \includegraphics[width=.95\linewidth]{figures/ablation_images/original.jpg}
%     \caption{original batch.}
% \end{subfigure}
% \includegraphics[width=.95\linewidth]{figures/ablation_images/grad_only.jpg}
% \includegraphics[width=.95\linewidth]{figures/ablation_images/1gpu.jpg}
% \includegraphics[width=.95\linewidth]{figures/ablation_images/4gpu_mean.jpg}
% \includegraphics[width=.95\linewidth]{figures/ablation_images/4gpu_reg.jpg}
% \caption{Towards the inversion of original batch of resolution $224\times224$ on ImageNet. (preliminary: will format into single rows.)}
% \label{fig:main_results_image}
% \end{figure*}

\begin{table*}[!t]
\centering
\begin{tabular}{c}
\includegraphics[width=.95\linewidth]{figures/ablation_images/original.jpg} \\
 \textbf{Original batch - ground truth}
 \vspace{1mm} \\
 \midrule
% \includegraphics[width=.95\linewidth]{figures/ablation_images/noise.jpg} \\
%   \textbf{Noise $\mathcal{N}(0, I)$ - starting point} \\
\includegraphics[width=.95\linewidth]{figures/ablation_images/grad_only.jpg} \\
 (a) $\underset{\mathbf{\hat{x}}}{\text{argmin }}{ {\mathcal{L_\text{grad}}(\mathbf{\hat{x}}; \nabla \mathbf{W})}} $ \\
\includegraphics[width=.95\linewidth]{figures/ablation_images/1gpu.jpg} \\
 (b) $\underset{\mathbf{\hat{x}}}{\text{argmin }}{ {\mathcal{L_\text{grad}}(\mathbf{\hat{x}}; \nabla \mathbf{W}) +  \mathcal{R_\text{fidelity}}(\mathbf{\hat{x})}}}$\\
\includegraphics[width=.95\linewidth]{figures/ablation_images/4gpu_mean.jpg} \\
 (c) $\underset{\mathbf{\hat{x}}}{\text{argmin }}{ {\mathcal{L_\text{grad}}(\mathbf{\hat{x}}; \nabla \mathbf{W}) +  \mathcal{R_\text{fidelity}}(\mathbf{\hat{x})}} + \mathcal{R_\text{mean.lazy}}(\mathbf{\hat{x})}}$ \\
% \includegraphics[width=.95\linewidth]{figures/ablation_images/4gpu_reg.jpg} \\
\includegraphics[width=.95\linewidth]{figures/ablation_images/4gpu_reg2.jpg} \\
  (d) $\underset{\mathbf{\hat{x}}}{\text{argmin }}{ {\mathcal{L_\text{grad}}(\mathbf{\hat{x}}; \nabla \mathbf{W}) +  \mathcal{R_\text{fidelity}}(\mathbf{\hat{x})}} + \mathcal{R_\text{mean.reg}}(\mathbf{\hat{x})}}$ \textbf{ - our final reconstruction}\\
\midrule

 \includegraphics[width=\columnwidth]{figures/sota_images/DLG.jpg} 
  \includegraphics[width=\columnwidth]{figures/sota_images/DI.jpg} \\
  DLG~\cite{zhu2019deep} \hspace{7cm}    DeepInversion~\cite{yin2020dreaming} \\
  \includegraphics[width=\columnwidth]{figures/sota_images/biggan_grad_final.jpg}  \includegraphics[width=\columnwidth]{figures/sota_images/fig_final.jpg} \\
  StyleGAN V2~\cite{karras2020analyzing}+BigGAN-deep~\cite{brock2018biggan} \hspace{7cm} FIG~\cite{geiping2020inverting} \\
%  \textbf{Synthesized inputs - previous work}
 \end{tabular}
 \caption{ImageNet batch gradient inversion on ResNet-50 ablation study on inversion loss and comparison with previous work.}
 \label{fig:against_sota}
 \end{table*}

==> figures/no_bn.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{c}
\includegraphics[width=.95\linewidth]{figures/ablation_images/original.jpg} \\
 \textbf{Original batch - ground truth}\\
\includegraphics[width=.95\linewidth]{figures/ablation_images/4gpu_reg2.jpg} \\
  (a) w/ original batch BN stats \\
\includegraphics[width=.95\linewidth]{figures/ablation_images/no_bn_v2.jpg} \\
  (b) w/o original batch BN stats \\
%  \textbf{Synthesized inputs - previous work}
 \end{tabular}
 \caption{ImageNet batch gradient inversion on ResNet-50 ablation study on inversion loss and comparison with previous work. MOCO V2 reverses out image patches and color contrast due to its contrastive learning.}
 \label{fig:no_bn}
 \end{table*}

==> figures/registration.tex <==
\begin{figure}[t]
\centering
\resizebox{0.85\linewidth}{!}{
\begingroup
\renewcommand*{\arraystretch}{0.3}
% \setlength\extrarowheight{-30pt}
\begin{tabular}{c|cc|c}
%original
\includegraphics[width=0.3\linewidth,clip,trim=5px 0 0 4px]{figures/registration/wo_reg.png} &
%ADI
\includegraphics[width=0.3\linewidth,clip,trim=5px 0 0 4px]{figures/registration/reg_to_gt.png} &
\includegraphics[width=0.3\linewidth,clip,trim=5px 0 0 4px]{figures/registration/w_reg.png} & \includegraphics[width=0.3\linewidth,clip,trim=5px 0 0 4px]{figures/registration/converged.png} 
\\
% $\frac{1}{S} \sum_{s \in S} \mathbf{\hat{x}_{s}}$ &
% $\frac{1}{S} \sum_{s \in S} \mathbf{F}_{\mathbf{\hat{x}_{s}} \rightarrow \mathbf{\hat{x}^*}}(\mathbf{\hat{x}_{s}})$ 
% &
% $\frac{1}{S} \sum_{s \in S} \mathbf{F}_{\mathbf{\hat{x}_{s}} \rightarrow \frac{1}{S} \sum_{s \in S}{\mathbf{\hat{x}_s}}}(\mathbf{\hat{x}_{s}})$ \\

(a) Pixel-wise mean & (b) Reg. to original & (c) Reg. to mean & (d) Upon Convergence \\

\end{tabular}
%
\endgroup
}
\caption{Impact of image registration on group consistency regularization. %\pmnote{this should be shown together with Figure 2. Also why don't we show registration in the end of optimization, I guess those images will look better.} 
}
\label{fig:registration}
\end{figure}

==> label_restore_old.tex <==









\iffalse
that consequentially forms a vector for each image $x_k$ as $\vec{s_k} = [s_1, s_2, ..., s_N]^{\text{T}} \in \mathbb{R}^N$, where only the ground truth label index gives a negative value, others being non-negative. Zhao \etal~\cite{zhao2020idlg} explored this rule for single image label restoration. %Danny - relocated this sentence back after some thoughts 
%Plugging Eqn.~\ref{eqn:s_vec} into Eqn.~\ref{eqn:lrestore_main} for batch size $K$,
Note that for a batch of images, this information is not yet observable - the given gradients is an averaged form of all images, leading to a batch-level indicator per class as:
% \begin{equation}
% \begin{aligned}
%   \underbrace{\nabla_{w_{m,n}}\mathcal{L}(\mathbf{x^*}, \mathbf{y^*})}_{\textrm{given in } \Delta \mathbf{W}_{\textbf{fc}}}  = \frac{1}{K} \sum_{k} \nabla_{z_{n, k}}\mathcal{L}(x_k, y_k) \times o_{m,k},
% \end{aligned}
% \end{equation}
% \noindent
% \begin{equation}
% \begin{aligned}
%   \underbrace{\nabla_{w_{m,n}}\mathcal{L}(\mathbf{x^*}, \mathbf{y^*})}_{\textrm{given in } \Delta \mathbf{W}_{\textbf{fc}}}  = \frac{1}{K} \sum_{k} \mathbf{W}^{\text{(FC)}}_{m, n, k},
% \end{aligned}
% \end{equation}
% \noindent
% which gives a batch-level indicator per class:
% \begin{equation}
% \begin{aligned}
%   s_{n,\text{batch}} &   = \sum_{k}
%     \frac{1}{K} \sum_{k} \overbrace{(\sum_{m} \nabla_{z_{n, k}}\mathcal{L}(x_k, y_k)\times o_{m,k})}^\textrm{$s_n$ of $\vec{s}$ of image $k$}
%   s_{n,\text{batch}} &   = 
%     \frac{1}{K} \sum_{k} \overbrace{(\sum_{m} \nabla_{z_{n, k}}\mathcal{L}(x_k, y_k)\times o_{m,k})}^\textrm{$s_n$ of $\vec{s}$ of image $k$}.
% \label{eqn:sbatch}
% \end{aligned}
% \end{equation}
% \noindent
\begin{equation}
\begin{aligned}
  s_{n} &   = \sum_{m} \big( \underbrace{
    \frac{1}{K} \sum_{k} \Delta \mathbf{W}^{\text{(FC)}}_{m, n, k}}_{\textrm{given in } \Delta \mathbf{W}_{\textbf{fc}}} \big) = 
    \frac{1}{K} \sum_{k} \underbrace{(\sum_{m} \Delta \mathbf{W}^{\text{(FC)}}_{m, n, k}\big)}_\textrm{$s_n$ of $\vec{s}$ for image $k$},
\label{eqn:sbatch}
\end{aligned}
\end{equation}
\noindent
%\AV{I spent a lot of time to decipher Eq. 6 to 9. I feel one reason is that $\nabla_{z_{i, k}}\mathcal{L}(x_k, y_k) \times o_{j,k}$ is just copy-pasted so many times. I think you should define $\nabla_{z_{i, k}}\mathcal{L}(x_k, y_k) \times o_{j,k}$ as a new variable in Eq. 5}
and consequentially forms a batch-level $s$ vector at:
\begin{equation}
  \vec{s}_{\text{batch}} = \sum_{m} \underbrace{\nabla_{w_{m,n}}\mathcal{L}(\mathbf{x^*}, \mathbf{y^*})}_{\textrm{given in } \Delta \mathbf{W}_{\textbf{fc}}} =   
    \frac{1}{K} \sum_{k} \vec{s}_k.
\label{eqn:sbatch}
\end{equation}
\noindent
As noted, $\vec{s}_{\text{batch}}$ is a linear super-position of $\vec{s_k}$ from all individual images $x_k$'s in the batch. Each $\vec{s_k}$ is an independent one-hot encoded vector, containing a single negative peak at the label index and positive otherwise, where heuristically encoded positions possess larger magnitudes $ |\vec{s}_{k,n_k^*}| >>  |\vec{s}_{k,n\neq n_k^*}|$ \footnote{\eg, $\frac{\sum_{n}|s_{k,n\neq n_k^*}|}{|s_{k, n_k^*}|} \rightarrow \frac{1}{999}$ on ImageNet training set upon convergence as $\mathbb{E}\big(\sum\limits_{m,n}{\nabla_{w_{m,n}}\mathcal{L}(\mathbf{x^*}, \mathbf{y^*})}\big) \rightarrow 0$, independent of networks.}. This leaves a negative sign mostly intact when the sum operation brings in positive values from other images. %As we can be notice, such efficacy diminishes as batch size increases, given more positive values from the batch accumulate. 

To further enable a more robust propagation of negative signs, we utilize column-wise minimum values instead of sums along the feature axis for the $\vec{s}_\text{batch}$ calculation: to have a sum along the feature dimension be negative, at least one of its positions has to be negative, but not vice versa. This further boosts up restoration accuracy, especially when batch size increases. Thus, we formulate the final label restoration algorithm for batch size $K$ as:
% \begin{equation}
% \begin{aligned}
%   \mathbf{\hat{y}} = argsort(\text{min}_{j \leq \# \text{features}}  \nabla_{w_{j,i}\in \mathbf{W}_{fc}}\mathcal{L}(\mathbf{x^*}, \mathbf{y^*}))[:K].
% \end{aligned}
% \end{equation}
%
\begin{equation}
\begin{aligned}
  \mathbf{\hat{y}} =  \text{arg sort}\big(\underset{ m}{\text{min }}  \nabla_{\mathbf{W}_{\textbf{fc}}}\mathcal{L}(\mathbf{x^*}, \mathbf{y^*})\big)[:K],
\end{aligned}
\label{eqn:label_restore}
\end{equation}
\noindent
with $m$ corresponding to the feature embedding dimension before the fully connected layer.
% \pmnote{the \# is not clear in equation}
The resulting $\mathbf{\hat{y}}$ supports Eqn.~\ref{eqn:lgrad} in subsequent $\mathbf{\hat{x}}$ optimization in pursuit for $\mathbf{x^*}$. One limitation of the current method assumes non-repeating labels in the batch, which generally holds for a randomly sampled batch of size $K$ that is much smaller than the number of classes at $1$K for ImageNet.

%\JK{Say something about reconstructed labels $\mathbf{\hat{y}}$ here?}\Danny{Agree - reorganizing}
Despite correct $\mathbf{y}^*$, descending into the global minimum for $\mathcal{L_\text{grad}}(\cdot)$ remains fairly challenging. The problem is over-constraint, 
%\JK{It's under-constraint, no?}\pmnote{over, because of having more parameters in the model than input pixels}
suffers information loss amid non-linearity and pooling layers, and has only one global optimal solution~\cite{geiping2020inverting,zhu2019deep}. We next introduce $\mathcal{R_\text{aux}}(\cdot)$ based on fidelity and group consistency regularization to assist with this optimization.
\fi

==> suppl_new.tex <==
\section*{Supplementary Materials - A}
We provide more experimental details in the following sections. 


\paragraph{$\mathcal{L}_{grad}$ cost function.} For the task of gradient matching, we study how the loss function affects optimization in Table~\ref{tb:loss_ablation_table}. 
We find $\ell_2$ loss outperforms cosine similarity~\cite{geiping2020inverting} for gradient matching. To this end, we compare the $\ell_2$ distance, percentage of gradient signs that matched, and the cosine similarity between the final optimized gradient and the ground truth gradient. It can be observed that an $\ell_2$ regularization results in stronger convergence for this task. 
\input{tables/cosine_table}


% \paragraph{Sensitivity to pre-processing.} Unlike our observations with DeepInversion, gradient matching is highly sensitive to pre-processing. A quick example is summarized in Table~\ref{}. We consequentially disabled all such steps.

% \input{tables/preprocessing}

\paragraph{Ablation studies qualitative results.}

We provide detailed visual comparison of the batch in ablation studies in Fig.~\ref{fig:ablation_imgs}.

\paragraph{Additional visual examples for privacy leakage.} We include more feature leakage examples in Fig.~\ref{fig:more_and_more}.


\paragraph{Insights \& Open challenges.} In our experiments, we observe the existence of several interesting facts of gradient inversion that may provide insights to future directions.
\begin{itemize}
    \item \textbf{Vanishing objects.} GradInverson can yield very similar images to original while come certain objects are missing as a whole. Interestingly this is in line as observation in latent code projection \etal~\cite{karras2020analyzing}.
    
    \item \textbf{Texts \& digits.} We observe gradient inversion reverses out existence of digits and letters, but not yet completely readable and remains private.
    
    \item \textbf{Human faces.} GradInversion still faces challenges with harder classes in ImageNet that involves human faces. Though reversing out segments of human faces, \eg mouths, eyes, and eyes, accurately relocating them in correct positions remain challenging. 
\end{itemize}


\input{figures/missing_objects}
% \noindent
% \textbf{With and without original BN statistics.}
% We next consider the case where without the original BN statistics and present the results in Table~\ref{tab:no_bn}. We observe an increased LPIPS at $0.642$, where we conjecture the BN statistic estimation may suffer differences when batch size is far beyond the original training batch size. However, DeepInversion$_{grad}$ still reveals image-level privacy, as shown in Fig.~\ref{fig:no_bn}. 

% \include{figures/no_bn}


\input{figures/main_results_image_ablation}

\input{figures/more_images}

==> tables/preprocessing.tex <==
\begin{table}[h]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{cc}
\toprule
Preproc. & \multicolumn{1}{c}{\textbf{$\nabla_{\mathbf{W}}\mathcal{L}(\mathcal{T}(x^*), \mathbf{y^*})$ vs. $\nabla_{\mathbf{W}}\mathcal{L}(\mathbf{x^*}, \mathbf{y^*})$}}\\
$\mathcal{T}(\cdot)$ & $\ell_2$ dist. $\downarrow$ \\
\midrule
None (upper bond) & $0$ \\
\midrule
brightness                  & 1.36 \\
saturation                  & 2.06 \\
contrast                    & 2.36 \\
cutout$_{.2}$               & 2.46 \\
% (\textbf{convergence$^*$})  & (\textbf{2.69}) \\
jitter$_{3}$                & 3.05 \\
jitter$_{5}$                & 3.21 \\
translation$_{.05}$         & 3.59 \\
cutout$_{.5}$               & 3.81 \\
translation$_{.125}$        & 3.84 \\
\midrule
$\mathcal{N}(0,\mathcal{I})$ (lower bond) & $8.62$ \\
\bottomrule
\end{tabular}}
\label{tab:vs_cos}
\caption{Gradient matching remains sensitive to preprocessing. We observe no improvements with augmentations for GradInversion, and observe they incur gradient mismatch even added to ground truth data.}
\label{tb:loss_ablation_table}
\end{table}
